DORA: Distributed Oracle Agreement with Simple Majority

Oracle networks feeding off-chain information to a blockchain are required to solve a distributed agreement problem since these networks receive information from multiple sources and at different times. We make a key observation that in most cases, the value obtained by oracle network nodes from multiple information sources are in close proximity. We define a notion of agreement distance and leverage the availability of a state machine replication (SMR) service to solve this distributed agreement problem with an honest simple majority of nodes instead of the conventional requirement of an honest super majority of nodes. Values from multiple nodes being in close proximity, therefore, forming a coherent cluster, is one of the keys to its efficiency. Our asynchronous protocol also embeds a fallback mechanism if the coherent cluster formation fails. Through simulations using real-world exchange data from seven prominent exchanges, we show that even for very small agreement distance values, the protocol would be able to form coherent clusters and therefore, can safely tolerate up to $1/2$ fraction of Byzantine nodes. We also show that, for a small statistical error, it is possible to choose the size of the oracle network to be significantly smaller than the entire system tolerating up to a $1/3$ fraction of Byzantine failures. This allows the oracle network to operate much more efficiently and horizontally scale much better.

==> discussion.tex <==
\section{Discussion}

\subsection{Data source failure \label{Se:dsfailure}}
\akcomment{some notes from here can go to the data source subsection and the rest can go to the extended version}
There are some other oracle models which are opaque about how the data is obtained by the node from a data source. While the probability that the data source itself is malicious may be very low in practice, a transient glitch in the data source is a real possibility that one must be able to accommodate while designing an oracle with strong safety guarantees. There are plenty of documented glitches and bugs ~\cite{seerene,slate}  which have resulted in stock exchanges coming to a grinding halt, or worse, emitting a price of a stock that is far from its actual value.

Imagine a model where one node is receiving its data from one data source. Even though an honest node is relaying the information that it received from the data source as-is to the oracle network, a glitch in the data source can make an honest node behave in a Byzantine fashion. Any oracle design that does not take into account the possibility of a Byzantine data source can not guarantee safety or liveness even in a $3f+1$ setting, where $f$ nodes of the oracle can turn Byzantine.  Imagine a network with $f$ Byzantine nodes and one Byzantine data source feeding to an honest node. This essentially breaches the limit of $f$ nodes behaving in a Byzantine fashion. The bounds of $[\hmin,\hmax]$ are tight and a single additional Byzantine observation can potentially introduce an unbounded error in the reported value.
Our design for \dora ensures that every node is listening to a sufficient number of data sources such that Byzantine behaviour of up to $f_d$ data sources can be tolerated.

When an oracle design does not mandate which data source a node should receive its data from, it is likely that many nodes would prefer receiving their data from a data source that is fast, considered relatively more reliable, or cheaper to subscribe to, etc. This can skew the distribution of nodes listening to data sources in favour of a few data sources. If one node is listening to only one data source and there is a data source that is feeding data to more than $f$ nodes, this data source becomes a single point of failure for the entire oracle network. Therefore, it is of utmost importance that every node not only listens to multiple data sources but the mapping of nodes to data sources is fairly uniform to provide higher resilience to the potential failure of a small set of data sources. Due to this consideration, in our oracle design, we mandate not only the minimum number of data sources that a node must receive its data from, but also a uniform random assignment of data sources generated via a VRF ({\em Verifiable Random Function}) that a node must listen to. Such a design results in one node listening to multiple data sources and also, every data source feeding to multiple nodes. Such uniform random assignment practically eliminates the possibility of  Byzantine data sources making an honest node behave in a Byzantine fashion.
\subsection{Mean v/s Median}

In \cref{Alg:defaultfallback}, we reach an agreement within the agreement distance \agreedist with only $f_c+1$ nodes. Since, it guarantees that there would be at least one honest observation within this set of $f_c+1$ observations, we decide to use mean to ensure that all the honest observations are definitely included in the final \svalue being proposed. Note that while using the median of  the coherent cluster would still be within the bounds $[\hmin-\agreedist,\hmax+\agreedist]$, a Byzantine majority within the set of $f_c+1$ observation may  move the \svalue slightly in the favor of the adversary. Using the mean allows honest observations to counterbalance byzantine observations, thereby mitigating a malicious movement of \svalue.

On the other hand, \cref{Alg:fallbackprotocol} uses the median as an aggregation since it offers maximum the robustness and resilience in the presence of corrupt data due to its breakdown point being $0.5$. Since there is no notion of the observations forming a coherent cluster in \cref{Alg:fallbackprotocol}, using the mean would allow an adversary to move \svalue in its favour arbitrarily and in an unbounded fashion.




==> figproto.tex <==
\begin{figure}

\caption{figure}
\label{Fi:doraccfallback}

\begin{tikzpicture}
\tikzstyle{ftriangle}=[regular polygon, regular polygon sides=3,draw,ultra thick,rotate=-90,anchor=south]
\tikzstyle{btriangle}=[regular polygon, regular polygon sides=3,draw,ultra thick,rotate=90,anchor=north]
\tikzstyle{bar}=[rectangle,draw,fill,minimum width=2cm, minimum height=0.1cm,rotate=90,anchor=north]


\node [draw, rectangle, rotate=90, anchor=north] (ds) {Data Sources};

\node[right=5mm of ds.south, draw, ultra thick, signal, signal from=west, minimum height=0.5cm] (ds2node) {  };
%\node[right=0.5cm of ds2node.east,bar] (fstage) {};
\draw let \p{ds2node}=(ds2node.east) in [ultra thick] (\x{ds2node}+3,\y{ds2node}-25) -- (\x{ds2node}+3,\y{ds2node}+25);
\node[right=0.2cm of ds2node.east, ftriangle ] (sendvalue) { \tiny{value}};

\draw let \p{sendvalue}=(sendvalue.north) in [ultra thick] (\x{sendvalue}+5,\y{sendvalue}-25) -- (\x{sendvalue}+5,\y{sendvalue}+25);
\node[right=1cm of sendvalue.north ,btriangle ] (proposal) {\tiny{Prop}};

\end{tikzpicture}
\end{figure}


==> refs.tex <==
\newcommand{\theoref}[1]{Thm.~\ref{The:#1}}
\newcommand{\theorefs}[2]{Thms.~\ref{The:#1} and~\ref{The:#2}}
\newcommand{\theorefsp}[3]{Thms.~\ref{The:#1}, \ref{The:#2}, and~\ref{The:#3}}
\newcommand{\lemref}[1]{Lem.~\ref{Lem:#1}}
\newcommand{\lemrefs}[2]{Lemmas~\ref{Lem:#1} and~\ref{Lem:#2}}
\newcommand{\lemrefsp}[3]{Lemmas~\ref{Lem:#1},~\ref{Lem:#2}, and~\ref{Lem:#3}}
\newcommand{\corref}[1]{Cor.~\ref{Cor:#1}}
\newcommand{\figref}[1]{Fig.~\ref{Fi:#1}}
\newcommand{\figrefs}[2]{Figs.~\ref{Fi:#1} and~\ref{Fi:#2}}
\newcommand{\defref}[1]{Defn.~\ref{De:#1}}
\newcommand{\defrefs}[2]{Defns.~\ref{De:#1} and~\ref{De:#2}}
\newcommand{\sdefref}[1]{Strawman Defn.~\ref{De:#1}}
\newcommand{\lineref}[1]{line~[\ref{Li:#1}]}
\newcommand{\linerefs}[2]{lines~[\ref{Li:#1}] and~[\ref{Li:#2}]}
\newcommand{\linerefsp}[3]{lines~[\ref{Li:#1}], [\ref{Li:#2}], and~[\ref{Li:#3}]}
\newcommand{\linerefspp}[4]{lines~[\ref{Li:#1}], [\ref{Li:#2}], [\ref{Li:#3}], and~[\ref{Li:#4}]}
\newcommand{\lineseqref}[2]{lines~[\ref{Li:#1}]--[\ref{Li:#2}]}
%\newcommand{\eqref}[1]{Eqn.~(\ref{Eq:#1})}
\newcommand{\eqrefs}[2]{Eqns.~(\ref{Eq:#1}) and~(\ref{Eq:#2})}
\newcommand{\eqrefsp}[3]{Eqns.~(\ref{Eq:#1}), (\ref{Eq:#2}), and~(\ref{Eq:#3})}
\newcommand{\eqrefspp}[4]{Eqns.~(\ref{Eq:#1}), (\ref{Eq:#2}), (\ref{Eq:#3}), and~(\ref{Eq:#4})}
\newcommand{\eqrefspOr}[3]{Eqns.~(\ref{Eq:#1}), (\ref{Eq:#2}), or~(\ref{Eq:#3})}
\newcommand{\eqrefsppOr}[4]{Eqns.~(\ref{Eq:#1}), (\ref{Eq:#2}), (\ref{Eq:#3}), or~(\ref{Eq:#4})}
\newcommand{\eqseqref}[2]{Eqns.~(\ref{Eq:#1})--(\ref{Eq:#2})}
\newcommand{\formref}[1]{Formula~(\ref{Eq:#1})}
\newcommand{\formrefs}[2]{Formulas~(\ref{Eq:#1}) and~(\ref{Eq:#2})}
\newcommand{\formrefsw}[2]{Formulas~(\ref{Eq:#1}) with~(\ref{Eq:#2})}
\newcommand{\formrefsp}[3]{Formulas~(\ref{Eq:#1}), (\ref{Eq:#2}), and~(\ref{Eq:#3})}
\newcommand{\formrefspp}[4]{Formulas~(\ref{Eq:#1}), (\ref{Eq:#2}), (\ref{Eq:#3}), and~(\ref{Eq:#4})}
\newcommand{\formrefspOr}[3]{Formulas~(\ref{Eq:#1}), (\ref{Eq:#2}), or~(\ref{Eq:#3})}
\newcommand{\formrefsppOr}[4]{Formulas~(\ref{Eq:#1}), (\ref{Eq:#2}), (\ref{Eq:#3}), or~(\ref{Eq:#4})}
\newcommand{\tableref}[1]{Tab.~\ref{Ta:#1}}
\newcommand{\tablerefs}[2]{Tabs.~\ref{Ta:#1} and~\ref{Ta:#2}}
\newcommand{\sectref}[1]{Section~\ref{Se:#1}}
\newcommand{\sectrefs}[2]{Sections~\ref{Se:#1} and~\ref{Se:#2}}
\newcommand{\sectrefsp}[3]{Sections~\ref{Se:#1}, \ref{Se:#2}, and~\ref{Se:#3}}
\newcommand{\sectseqref}[2]{Sections~\ref{Se:#1}--\ref{Se:#2}}
\newcommand{\appref}[1]{Appendix~\ref{App:#1}}
\newcommand{\apprefs}[2]{Apps.~\ref{App:#1} and~\ref{App:#2}}
\newcommand{\exref}[1]{Ex.~\ref{Exa:#1}}
\newcommand{\exrefs}[2]{Exs.~\ref{Exa:#1} and~\ref{Exa:#2}}
\newcommand{\exrefsp}[3]{Exs.~\ref{Exa:#1}, \ref{Exa:#2}, and~\ref{Exa:#3}}
\newcommand{\exrefspp}[4]{Exs.~\ref{Exa:#1}, \ref{Exa:#2}, \ref{Exa:#3}, and~\ref{Exa:#4}}
\newcommand{\ruleref}[1]{Rule~(\ref{Rule:#1})}
\newcommand{\rulerefs}[2]{Rules~(\ref{Rule:#1}) and~(\ref{Rule:#2})}
\newcommand{\rulerefsp}[3]{Rules~(\ref{Rule:#1}), (\ref{Rule:#2}), and~(\ref{Rule:#3})}
\newcommand{\rulerefspp}[4]{Rules~(\ref{Rule:#1}), (\ref{Rule:#2}), (\ref{Rule:#3}), and~(\ref{Rule:#4})}
\newcommand{\prodref}[1]{Prod.~(\ref{Prod:#1})}
\newcommand{\prodrefs}[2]{Prods.~(\ref{Prod:#1}) and~(\ref{Prod:#2})}
\newcommand{\prodrefsp}[3]{Prods.~(\ref{Prod:#1}), (\ref{Prod:#2}), and~(\ref{Prod:#3})}
\newcommand{\prodrefspp}[4]{Prods.~(\ref{Prod:#1}), (\ref{Prod:#2}), (\ref{Prod:#3}), and~(\ref{Prod:#4})}
\newcommand{\constraintref}[1]{Constraint~(\ref{Eq:#1})}
\newcommand{\constraintrefs}[2]{Constraints~(\ref{Eq:#1}) and~(\ref{Eq:#2})}
\newcommand{\constraintrefsp}[3]{Constraints~(\ref{Eq:#1}), (\ref{Eq:#2}), and~(\ref{Eq:#3})}
\newcommand{\itemref}[1]{item~\ref{It:#1}}
\newcommand{\itemrefs}[2]{items~\ref{It:#1} and~\ref{It:#2}}
\newcommand{\itemrefsp}[3]{items~\ref{It:#1}, \ref{It:#2}, and~\ref{It:#3}}
\newcommand{\itemrefspp}[4]{items~\ref{It:#1}, \ref{It:#2}, \ref{It:#3}, and~\ref{It:#4}}
\newcommand{\itemseqref}[2]{items~[\ref{It:#1}]--[\ref{It:#2}]}
\newcommand{\Itemref}[1]{Item~\ref{It:#1}}
\newcommand{\Itemrefs}[2]{Items~\ref{It:#1} and~\ref{It:#2}}
\newcommand{\Itemrefsp}[3]{Items~\ref{It:#1}, \ref{It:#2}, and~\ref{It:#3}}
\newcommand{\Itemrefspp}[4]{Items~\ref{It:#1}, \ref{It:#2}, \ref{It:#3}, and~\ref{It:#4}}
\newcommand{\Itemseqref}[2]{Items~[\ref{It:#1}]--[\ref{It:#2}]}
\newcommand{\algref}[1]{Alg.~\ref{Alg:#1}}
\newcommand{\algline}[1]{(Line~\ref{Line:#1})}
\newcommand{\alglines}[2]{(Lines~\ref{Line:#1}--\ref{Line:#2})}
\newcommand{\alglinestwo}[2]{(Lines~\ref{Line:#1} and~\ref{Line:#2})}
\newcommand{\algrefs}[2]{Algs.~\ref{Alg:#1} and~\ref{Alg:#2}}
\newcommand{\algrefsp}[3]{Algs.~\ref{Alg:#1}, \ref{Alg:#2}, and~\ref{Alg:#3}}
\newcommand{\algrefspp}[4]{Algs.~\ref{Alg:#1}, \ref{Alg:#2}, \ref{Alg:#3}, and~\ref{Alg:#4}}
\newcommand{\assumptionref}[1]{Assumption~(\ref{Assumption:#1})}
\newcommand{\assumptionrefs}[2]{Assumptions~(\ref{Assumption:#1}) and~(\ref{Assumption:#2})}
\newcommand{\footnoteref}[1]{footnote~\ref{Footnote:#1}}
\newcommand{\footnoterefs}[2]{footnote~\ref{Footnote:#1} and~\ref{Footnote:#2}}
\newcommand{\obnref}[1]{Obs.~\ref{obn:#1}}
\newcommand{\obnrefs}[2]{Obs.~\ref{obn:#1} and~\ref{obn:#2}}
\newcommand{\propref}[1]{Prop.~\ref{prop:#1}}

